Instance-wise Prompt Tuning for Pretrained Language Models

Prompt Learning has recently gained great popularity in bridging the gap between pretraining tasks and various downstream tasks. It freezes Pretrained Language Models (PLMs) and only tunes a few task-related parameters (prompts) for downstream tasks, greatly reducing the cost of tuning giant models. The key enabler of this is the idea of querying PLMs with task-specific knowledge implicated in prompts. This paper reveals a major limitation of existing methods that the indiscriminate prompts for all input data in a task ignore the intrinsic knowledge from input data, resulting in sub-optimal performance. We introduce Instance-wise Prompt Tuning (IPT), the first prompt learning paradigm that injects knowledge from the input data instances to the prompts, thereby providing PLMs with richer and more concrete context information. We devise a series of strategies to produce instance-wise prompts, addressing various concerns like model quality and cost-efficiency. Across multiple tasks and resource settings, IPT significantly outperforms task-based prompt learning methods, and achieves comparable performance to conventional finetuning with only 0.5% - 1.5% of tuned parameters.

==> 3.problem.tex <==
\section{Instance-wise prompting problem}
\subsection{Problem Setup and Notation}
Following the "text-to-text" pattern of T5~\cite{raffel2019exploring} and prompt tuning~\cite{lester2021power}, we cast all tasks as text generation, and modeling the classification process as probability of an output class given some input, $Pr(y\|x)$, where x is a series of input tokens and y is a sequence of tokens that represent the class label of x. 

For a given dataset $\mathbf{X} =\{x_1, x_2, \cdots, x_m\}$, each $x_i$ in $\mathbf{X}$ can be tokenized into a sequence of n tokens $x_i = \{x_{i_1}, x_{i_2}, \cdots, x_{i_n}\}$. For a given target set $\mathbf{Y} = \{y_1, y_2, \cdots, y_m\}$, each $y_i$ in $\mathbf{Y}$ is a sequence of tokens that represent a class label for corresponding $x_i$ in $\mathbf{X}$. The basic PLM is parameterized by the weights of $\theta$. 

To perform instance-wise prompting, we produce instance-wise prompts by strategy $\mathbf{G_{\omega}}$ which is parameterized by $\omega$. Given data $x_i$, \sys firstly generate a series of instance-wise prompt tokens $t_i = \{t_{i_1}, t_{i_2}, \cdots, t_{i_k}\}$ for $x_i$ by:
\begin{small}
\begin{equation}
    t_i = \mathbf{G_{\theta}}(x_i),
    \label{generator}
\end{equation}
\end{small}
where $k$ is a hyper-parameter that denotes the number of prompt tokens. The prompt is then concatenated to the input data forming a prompted instance representation $[t_i,x_i]$ for downstream tasks. 

The goal of \sys is to maximize the likelihood of correct $y_i$ in $\mathbf{Y}$ for $x_i$, $Pr_{\theta, \omega}(y_i\|[t_i,x_i])$, while keeping the PLMs' parameters $\theta$ fixed, and only applying gradient updates to $\omega$. 

\subsection{Motivating Analysis}
\label{motivation}
% \begin{figure}[tpb]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figure/observation.pdf}
%     % \vspace{-4mm}
%     \caption{The Observation on instance-wise prompts's effects.}
%     \label{observation}
%     % \vspace{-4mm}
% \end{figure}

One major difference of \sys and existing works is the instance-wise prompting manner. To better introduce our work, we first perform an observational study of instance-wise prompting on SuperGLUE dataset. 
% The analysis provides insights to building \sys. 

\para{Data Difference Matters.}
One important characteristics of existing methods outlined in the previous section is the shared and task-based prompt space. Generally, they ignore the difference in syntax and semantics of input data, and assign a common trainable embedding for all input data. 
Despite specific tasks have different requirements on language models' capacities, the heart of language tasks lies in natural language understanding, which is closely relative to the specific content of input data. 
For example, though true-false problems generally demand inference capability for language models, the correct answers are implicated in specific sentences. 
We suspect that a shared representations may hinder PLMs' ability of capturing linguistic features according to linguistic discrepancies. Given this concern, we experiment with Roberta models and Prompt Tuning~\cite{lester2021power} in the following settings: (1). Instance-wise prompt space - Instead of initializing a task-based unifying soft prompt, we initialize our prompt aligned with Roberta's vocabulary tables, which means that we initialize prompt in the token level; (2). Instance-wise training - We simply truncating each instance by 100 tokens and prompting in a instance manner by querying tokens in the soft prompt space mentioned in (1). Except for (1) and (2), we keep other settings identical with Prompt Tuning (e.g., freezing PLM's parameters and simply tuning on prompts). We perform our experiment on two open benchmark from SuperGLUE: BoolQ and CB, and we report the results in~\ref{observation}. Surprisingly, we find that by only modifying the prompt format of Prompt Tuning to a instance-wise manner and keeping other settings identical with Prompt Tuning, the instance-wise variant of Prompt Tuning successively outperforms Prompt Tuning in the two datasets. The results demonstrates that instance-wise knowledge is generally beneficial for stimulating PLMs for downstream tasks. 

\subsection{Design Choice} 
The observation in Sec.~\ref{motivation} provide insights into important components of an flexible prompt model, which we take as design choices for our model. The model should (1) generate instance-wise prompts for input data; (2) For each instance, the prompt could implicate data-wise intrinsic knowledge that can better stimulate PLMs for downstream tasks in a lightweight way. Next we develop a easy-to-use model that satisfies these conditions. 

